Spatial and Kinematic Distributions of Transition Populations in Intermediate Redshift Galaxy Clusters

We analyze the spatial and velocity distributions of confirmed members in five massive clusters of galaxies at intermediate redshift (0.5 < z < 0.9) to investigate the physical processes driving galaxy evolution. Based on spectral classifications derived from broad- and narrow-band photometry, we define four distinct galaxy populations representing different evolutionary stages: red sequence (RS) galaxies, blue cloud (BC) galaxies, green valley (GV) galaxies, and luminous compact blue galaxies (LCBGs). For each galaxy class, we derive the projected spatial and velocity distribution and characterize the degree of subclustering. We find that RS, BC, and GV galaxies in these clusters have similar velocity distributions, but that BC and GV galaxies tend to avoid the core of the two z~0.55 clusters. GV galaxies exhibit subclustering properties similar to RS galaxies, but their radial velocity distribution is significantly platykurtic compared to the RS galaxies. The absence of GV galaxies in the cluster cores may explain their somewhat prolonged star-formation history. The LCBGs appear to have recently fallen into the cluster based on their larger velocity dispersion, absence from the cores of the clusters, and different radial velocity distribution than the RS galaxies. Both LCBG and BC galaxies show a high degree of subclustering on the smallest scales, leading us to conclude that star formation is likely triggered by galaxy-galaxy interactions during infall into the cluster.

==> tab_velocity_distrib_hist.tex <==
%% filename = tab_velocity_distrib_hist.dat
%% creator  = tab_velocity_distrib_hist.pro
%% date     = Wed Sep 25 21:36:06 2013
%% column1  = cluster
%% column2  = subset
%% column3  = N_members
%% column4  = delta_v [km/s]
%% column5  = scale
%% column6  = skewness
%% column7  = kurtosis
\wov & RSX & 118 & $91$ & $\pm$ & $122$ & $1262$ & $\pm$ & $72$ & $0.2$ & $\pm$ & $0.2$ & $ -0.5$ & $\pm$ & $0.2$ \\
\wov & GV & 26 & $-59$ & $\pm$ & $266$ & $1266$ & $\pm$ & $126$ & $0.1$ & $\pm$ & $0.3$ & $ -1.3$ & $\pm$ & $0.3$ \\
\wov & BCX & 44 & $-91$ & $\pm$ & $203$ & $1299$ & $\pm$ & $103$ & $0.1$ & $\pm$ & $0.2$ & $ -1.1$ & $\pm$ & $0.2$ \\
\wov & LCBG & 32 & $-604$ & $\pm$ & $266$ & $1376$ & $\pm$ & $182$ & $0.7$ & $\pm$ & $0.4$ & $ 0.1$ & $\pm$ & $1.1$ \\
~\\
\woi & RSX & 92 & $-135$ & $\pm$ & $162$ & $1462$ & $\pm$ & $113$ & $-0.2$ & $\pm$ & $0.2$ & $ -0.5$ & $\pm$ & $0.3$ \\
\woi & GV & 16 & $254$ & $\pm$ & $540$ & $1829$ & $\pm$ & $272$ & $0.1$ & $\pm$ & $0.3$ & $ -1.3$ & $\pm$ & $0.4$ \\
\woi & BCX & 28 & $33$ & $\pm$ & $234$ & $1130$ & $\pm$ & $136$ & $-0.2$ & $\pm$ & $0.3$ & $ -0.9$ & $\pm$ & $0.4$ \\
\woi & LCBG & 24 & $303$ & $\pm$ & $493$ & $2057$ & $\pm$ & $220$ & $0.1$ & $\pm$ & $0.3$ & $ -1.3$ & $\pm$ & $0.2$ \\
~\\
\woviii & RSX & 20 & $-60$ & $\pm$ & $166$ & $682$ & $\pm$ & $134$ & $0.1$ & $\pm$ & $0.4$ & $ -0.3$ & $\pm$ & $0.6$ \\
\woviii & GV & 4 & $651$ & $\pm$ & $781$ & $1037$ & $\pm$ & $594$ & $-0.4$ & $\pm$ & $0.4$ & $ -2.0$ & $\pm$ & $0.3$ \\
\woviii & BCX & 17 & $-212$ & $\pm$ & $164$ & $641$ & $\pm$ & $116$ & $-0.0$ & $\pm$ & $0.4$ & $ -0.8$ & $\pm$ & $0.5$ \\
\woviii & LCBG & 5 & $854$ & $\pm$ & $1032$ & $995$ & $\pm$ & $994$ & $0.0$ & $\pm$ & $0.5$ & $ -2.1$ & $\pm$ & $0.6$ \\
~\\
\wovii & RSX & 80 & $-79$ & $\pm$ & $122$ & $1039$ & $\pm$ & $83$ & $-0.0$ & $\pm$ & $0.2$ & $ -0.6$ & $\pm$ & $0.3$ \\
\wovii & GV & 18 & $297$ & $\pm$ & $285$ & $1063$ & $\pm$ & $170$ & $0.0$ & $\pm$ & $0.4$ & $ -1.0$ & $\pm$ & $0.5$ \\
\wovii & BCX & 37 & $-297$ & $\pm$ & $189$ & $996$ & $\pm$ & $139$ & $0.5$ & $\pm$ & $0.3$ & $ -0.3$ & $\pm$ & $0.6$ \\
\wovii & LCBG & 16 & $751$ & $\pm$ & $392$ & $1407$ & $\pm$ & $258$ & $-0.5$ & $\pm$ & $0.4$ & $ -0.6$ & $\pm$ & $0.8$ \\
~\\
\wx & RSX & 7 & $-195$ & $\pm$ & $249$ & $524$ & $\pm$ & $201$ & $0.5$ & $\pm$ & $0.5$ & $ -1.2$ & $\pm$ & $0.6$ \\
\wx & GV & 2 & $-102$ & $\pm$ & $\cdots$ & $570$ & $\pm$ & $\cdots$ & $0.0$ & $\pm$ & $\cdots$ & $ -2.8$ & $\pm$ & $\cdots$ \\
\wx & BCX & 17 & $103$ & $\pm$ & $334$ & $1143$ & $\pm$ & $208$ & $0.3$ & $\pm$ & $0.4$ & $ -0.7$ & $\pm$ & $0.5$ \\
\wx & LCBG & 16 & $-78$ & $\pm$ & $377$ & $1335$ & $\pm$ & $245$ & $-0.5$ & $\pm$ & $0.3$ & $ -0.9$ & $\pm$ & $0.5$ \\

